Algorithms for geometrical operations with NURBS surfaces

The aim of the paper is to show algorithms for geometrical manipulations on NURBS surfaces. These include generating NURBS surfaces that pass through given points, calculating the minimum distance to a point and include line to surface and surface to surface intersections.

==> settings/myheadings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % myheadings.tex
% %
% % 	requires:		\usepackage{scrpage2}
% % 				\usepackage{setspace}
% %

%%% Headings
%\pagestyle{headings}
\automark[chapter]{section}
\pagestyle{scrheadings}
% \rehead{\chaptermark}
\chead{}
\rohead[]{\pagemark}
%\rohead{\pagemark}
%\lohead{\rightmark}
\lohead{\rightmark}
\rehead{\leftmark}
% \lehead{}
\lehead{\pagemark}
\lefoot{}
\cefoot[]{}
\cofoot[]{}
% \rofoot[\pagemark]{\pagemark}
\rofoot[]{}
\setheadsepline{1pt}

%%% Vertical offset of chapters (standard is 1.8)
\renewcommand*{\chapterheadstartvskip}{\vspace{2.2\baselineskip}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 

